SAD: Segment Any RGBD

The Segment Anything Model (SAM) has demonstrated its effectiveness in segmenting any part of 2D RGB images. However, SAM exhibits a stronger emphasis on texture information while paying less attention to geometry information when segmenting RGB images. To address this limitation, we propose the Segment Any RGBD (SAD) model, which is specifically designed to extract geometry information directly from images. Inspired by the natural ability of humans to identify objects through the visualization of depth maps, SAD utilizes SAM to segment the rendered depth map, thus providing cues with enhanced geometry information and mitigating the issue of over-segmentation. We further include the open-vocabulary semantic segmentation in our framework, so that the 3D panoptic segmentation is fulfilled. The project is available on https://github.com/Jun-CEN/SegmentAnyRGBD.

==> Segment any RGBD/exp.tex <==
\begin{table}[t]
    \centering
    \caption{\textbf{Evaluation results on the FlyingThings3D and KITTI datasets.} $\mathit{Self}$ means self-supervised, $\mathit{Full}$ means fully-supervised. All approaches are (at least) trained on FlyingThings3D. On KITTI, $\mathit{Self}$ and $\mathit{Full}$ refer to the respective models trained on FlyingThings3D that is directly evaluated on KITTI, while \textit{Self+Self} means the model is firstly trained on FlyingThings3D with self-supervision, then fine-tuned on KITTI  with self-supervision as well. \textit{Full+Self} means the model is trained with full supervision on FlyingThings3D, then fine-tuned on KITTI with self-supervision. ICP~\cite{besl1992method}, FGR~\cite{zhou2016fast}, and CPD~\cite{myronenko2010point} are traditional method that does not require training. Our model outperforms all baselines by a large margin on all metrics}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|l|c|cccc|cc}
        %\cline{2-9}
        \hline\noalign{\smallskip}
        Dataset &Method         & Sup.  & EPE3D(m)$\downarrow$           & Acc3DS$\uparrow$          & Acc3DR$\uparrow$          & Outliers3D$\downarrow$      & EPE2D(\textit{px})$\downarrow$           & Acc2D$\uparrow$           \\
        \noalign{\smallskip}\hline\noalign{\smallskip}
    \multirow{9}{*}{Flyingthings3D}&ICP(rigid)~\cite{besl1992method} & $\mathit{Self}$& 0.4062          & 0.1614          & 0.3038          & 0.8796          & 23.2280         & 0.2913          \\
        &FGR(rigid)~\cite{zhou2016fast}        &$\mathit{Self}$& 0.4016  & 0.1291   & 0.3461  & 0.8755  & 28.5165  & 0.3037    \\
        &CPD(non-rigid)~\cite{myronenko2010point} &$\mathit{Self}$& 0.4887  & 0.0538   & 0.1694  & 0.9063  & 26.2015  & 0.0966    \\
        &PointPWC-Net   & $\mathit{Self}$& \textbf{0.1213} & \textbf{0.3239} & \textbf{0.6742} & \textbf{0.6878} & \textbf{6.5493} & \textbf{0.4756} \\
        \noalign{\smallskip}\cline{2-9}\noalign{\smallskip}
        &FlowNet3D~\cite{liu2019flownet3d}     &$\mathit{Full}$& 0.1136          & 0.4125          & 0.7706          & 0.6016          & 5.9740          & 0.5692          \\
        &SPLATFlowNet~\cite{su2018splatnet}   &$\mathit{Full}$& 0.1205          & 0.4197          & 0.7180          & 0.6187          & 6.9759          & 0.5512          \\
        &original BCL~\cite{gu2019hplflownet}   &$\mathit{Full}$& 0.1111          & 0.4279          & 0.7551          & 0.6054          & 6.3027          & 0.5669          \\
        &HPLFlowNet~\cite{gu2019hplflownet}     &$\mathit{Full}$& 0.0804          & 0.6144          & 0.8555          & 0.4287 & 4.6723          & 0.6764          \\
        &PointPWC-Net   &$\mathit{Full}$& \textbf{0.0588} & \textbf{0.7379} & \textbf{0.9276} & \textbf{0.3424}  & \textbf{3.2390} & \textbf{0.7994} \\
        \noalign{\smallskip}\hline\noalign{\smallskip}
    \multirow{11}{*}{KITTI}&ICP(rigid)~\cite{besl1992method}        &$\mathit{Self}$& 0.5181          & 0.0669          & 0.1667          & 0.8712          & 27.6752         & 0.1056          \\
        &FGR(rigid)~\cite{zhou2016fast}        &$\mathit{Self}$& 0.4835  & 0.1331   & 0.2851  & 0.7761  & 18.7464  & 0.2876    \\
        &CPD(non-rigid)~\cite{myronenko2010point}        &$\mathit{Self}$& 0.4144  & 0.2058      & 0.4001 & 0.7146 & 27.0583 & 0.1980 \\
        &PointPWC-Net(w/o ft) &$\mathit{Self}$& \textit{0.2549} & \textit{0.2379} & \textit{0.4957} & \textit{0.6863} & \textit{8.9439} & \textit{0.3299} \\
        &PointPWC-Net(w/ ft) &$\mathit{Self + Self}$& \textbf{0.0461} & \textbf{0.7951} & \textbf{0.9538} & \textbf{0.2275} & \textbf{2.0417} & \textbf{0.8645} \\
        \noalign{\smallskip}\cline{2-9}\noalign{\smallskip}
        &FlowNet3D~\cite{liu2019flownet3d}   &$\mathit{Full}$& 0.1767          & 0.3738          & 0.6677          & 0.5271          & 7.2141          & 0.5093          \\
        &SPLATFlowNet~\cite{su2018splatnet} &$\mathit{Full}$& 0.1988          & 0.2174          & 0.5391          & 0.6575          & 8.2306          & 0.4189          \\
        &original BCL~\cite{gu2019hplflownet} &$\mathit{Full}$& 0.1729          & 0.2516          & 0.6011          & 0.6215          & 7.3476          & 0.4411          \\
        &HPLFlowNet~\cite{gu2019hplflownet}   &$\mathit{Full}$& 0.1169 & 0.4783          & 0.7776 & 0.4103          & 4.8055          & 0.5938          \\
        &PointPWC-Net(w/o ft) &$\mathit{Full}$& \textit{0.0694}  & \textit{0.7281} & \textit{0.8884} & \textit{0.2648} & \textit{3.0062} & \textit{0.7673} \\
        &PointPWC-Net(w/ ft) &$\mathit{Full+Self}$& \textbf{0.0430} & \textbf{0.8175} & \textbf{0.9680} & \textbf{0.2072} & \textbf{1.9022} & \textbf{0.8669} \\
        \noalign{\smallskip}\hline
    \end{tabular}
    \label{tab:results}
    }
\end{table}


In this section, we train and evaluate our PointPWC-Net on the FlyingThings3D dataset~\cite{mayer2016large} with the supervised loss and the self-supervised loss, respectively. Then, we evaluate the generalization ability of our model by first applying the model on the real-world KITTI Scene Flow dataset~\cite{Menze2018JPRS,Menze2015ISA} \textit{without any fine-tuning}. Then, with the proposed self-supervised losses, we further fine-tune our pre-trained model on the KITTI dataset to study the best performance we could obtain without supervision. Besides, we also compare the runtime of our model with previous work. Finally, we conduct ablation studies to analyze the contribution of each part of the model and the loss function.

\noindent \textbf{Implementation Details.} We build a 4-level feature pyramid from the input point cloud. The weights $\alpha$ are set to be $\alpha_0=0.02$, $\alpha_1=0.04$, $\alpha_2=0.08$, and $\alpha_3=0.16$, with weight decay $0.0001$.% for both supervised learning and self-supervised learning. 
The scale factor $\beta$ in self-supervised learning are set to be $\beta_1=1.0$, $\beta_2=1.0$, and $\beta_3=0.3$. We train our model starting from a learning rate of $0.001$ and reducing by half every 80 epochs. All the hyperparameters are set using the validation set of FlyingThings3D with 8,192 points in each input point cloud.

\noindent \textbf{Evaluation Metrics.} For fair comparison, we adopt the evaluation metrics that are used in \cite{gu2019hplflownet}. Let $SF_{\Theta}$ denote the predicted scene flow, and $SF_{GT}$ be the ground truth scene flow. The evaluate metrics are computed as follows:

\noindent $\bullet$ \textit{EPE3D(m)}: $\norm{SF_{\Theta}-SF_{GT}}_2$ averaged over each point in meters.

\noindent $\bullet$ \textit{Acc3DS}: the percentage of points with \textit{EPE3D} $< 0.05m$ or relative error $<5\%$.

\noindent $\bullet$ \textit{Acc3DR}: the percentage of points with \textit{EPE3D} $< 0.1m$ or relative error $<10\%$.

\noindent $\bullet$ \textit{Outliers3D}: the percentage of points with \textit{EPE3D}$>0.3m$ or relative error $>10\%$.

\noindent $\bullet$ \textit{EPE2D(px)}: 2D end point error obtained by projecting point clouds back to the image plane.

\noindent $\bullet$ \textit{Acc2D}: the percentage of points whose \textit{EPE2D} $< 3px$ or relative error $<5\%$.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{images/fly_compare.pdf}
    \caption{\textbf{Results on the FlyingThings3D dataset.} In (a), 2 point clouds PC1 and PC2 are presented in Magenta and Green, respectively. In (b-f), PC1 is warped to PC2 based on the (computed) scene flow. (b) shows the ground truth; (c) Results from FGR(rigid)~\cite{zhou2016fast}; (d) Results from CPD(non-rigid)~\cite{myronenko2010point}; (e) Results from PointPWC-Net(\textit{Full}); (f) Results from PointPWC-Net(\textit{Self}). Red ellipses indicate locations with significant non-rigid motion. Enlarge images for better view. (Best viewed in color)}
    \label{fig:res_flyingthings3d}
\end{figure}

\subsection{Supervised Learning}
First we conduct experiments with supervised loss. To our knowledge, there is no publicly available large-scale real-world dataset that has scene flow ground truth from point clouds (The input to the KITTI scene flow benchmark is 2D), thus we train our PointPWC-Net on the synthetic Flyingthings3D dataset, following~\cite{gu2019hplflownet}. Then, the pre-trained model is directly evaluated on KITTI Scene Flow 2015 dataset without any fine-tuning. % to demonstrate the generalization ability of our model.


\noindent \textbf{Train and Evaluate on FlyingThings3D.}
The FlyingThings3D training dataset includes 19,640 pairs of point clouds, and the evaluation dataset includes 3,824 pairs of point clouds. Our model takes $n=8,192$ points in each point cloud. We first train the model with $\frac{1}{4}$ of the training set(4,910 pairs), and then fine-tune it on the whole training set, to speed up training.

Table~\ref{tab:results} shows the quantitative evaluation results on the Flyingthings3D dataset. 
%We compare our method with FlowNet3D~\cite{liu2019flownet3d}, SPLATFlowNet~\cite{su2018splatnet}, original BCL~\cite{gu2019hplflownet}, and HPLFlowNet~\cite{gu2019hplflownet}. 
Our method outperforms all the methods on all metrics by a large margin. %Compared to FlowNet3D, our cost volume layer is able to capture the motion information better. 
Comparing to SPLATFlowNet, original BCL, and HPLFlowNet, our method avoids the preprocessing step of building a permutohedral lattice from the input. Besides, our method outperforms HPLFlowNet on \textit{EPE3D} by $\mathit{26.9\%}$. And, we are the only method with \textit{EPE2D} under 4px, which improves over HPLFlowNet by $\mathit{30.7\%}$. See Fig.\ref{fig:res_flyingthings3d}(e) for example results.

\noindent \textbf{Evaluate on KITTI w/o Fine-tune.} To study the generalization ability of our PointPWC-Net, we directly take the model trained using FlyingThings3D and evaluate it on KITTI Scene Flow 2015~\cite{Menze2015ISA,Menze2018JPRS} \textit{without any fine-tuning}. KITTI Scene Flow 2015 consists of 200 training scenes and 200 test scenes. To evaluate our PointPWC-Net, we use  ground truth labels and trace raw point clouds associated with the frames, following \cite{liu2019flownet3d,gu2019hplflownet}. Since no point clouds and ground truth are provided on test set, we evaluate on all 142 scenes in the training set with available point clouds. We remove ground points with height $<0.3m$ following \cite{gu2019hplflownet} for fair comparison with previous methods. 

From Table~\ref{tab:results}, our PointPWC-Net outperforms all the state-of-the-art methods, which demonstrates the generalization ability of our model. For \textit{EPE3D}, our model is the only one below $10cm$, which improves over HPLFlowNet by $\mathit{40.6\%}$. For \textit{Acc3DS}, our method outperforms both FlowNet3D and HPLFlowNet by $\mathit{35.4\%}$ and $\mathit{25.0\%}$ respectively. See Fig.\ref{fig:res_kitti}(e) for example results. 

\begin{table}[t]
    \centering
    \caption{\textbf{Model design.} A learnable cost volume preforms much better than inner product cost volume used in PWC-Net~\cite{sun2018pwc}. Using our cost volume instead of the MLP+Maxpool used in FlowNet3D's flow embedding layer improves performance by $20.6\%$. Compared to no warping, the warping layer improves the performance by $40.2\%$}
    \begin{tabular}{l|c|c}
    \hline\noalign{\smallskip}
    Component                      & Status & EPE3D(m)$\downarrow$ \\
    \noalign{\smallskip}\hline\noalign{\smallskip}
    \multirow{3}{*}{Cost Volume}   & PWC-Net~\cite{sun2018pwc}& 0.0821 \\
                                   & MLP+Maxpool(learnable)~\cite{liu2019flownet3d}& 0.0741 \\
                                   & Ours(learnable) &  \textbf{0.0588} \\
    \noalign{\smallskip}\hline\noalign{\smallskip}
    \multirow{2}{*}{Warping Layer} & w/o      & 0.0984 \\
                                   & w    & \textbf{0.0588} \\
    \noalign{\smallskip}\hline
    \end{tabular}
    \label{tab:modeldesign}
\end{table}

\subsection{Self-supervised Learning}
Acquiring or annotating dense scene flow from real-world 3D point clouds is very expensive, so it would be interesting to evaluate the performance of our self-supervised approach. %study how to estimate scene flow given two input point clouds without ground truth. Based on the observation that the input point clouds should have structure or shape correspondences, %we propose to use Chamfer distance along with smoothness constraint and Laplac
%ian regularization as loss function to estimate scene flow. 
We train our model using the same procedure as in supervised learning, i.e. first train the model with one quarter of the training dataset, then fine-tune with the whole training set. Table~\ref{tab:results} gives the quantitative results on PointPWC-Net with self-supervised learning. We compare our method with ICP(rigid)~\cite{besl1992method}, FGR(rigid)~\cite{zhou2016fast} and CPD(non-rigid)~\cite{myronenko2010point}. Because traditional point registration methods are not trained with ground truth, we can view them as self/un-supervised methods. 



\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{images/kitti_compare.pdf}
    \caption{\textbf{Results on the KITTI Scene Flow 2015 dataset.} In (a), 2 point clouds PC1 and PC2 are presented in Magenta and Green, respectively. In (b-f), PC1 is warped to PC2 based on the (computed) scene flow. (b) shows the ground truth; (c) Results from FGR(rigid)~\cite{zhou2016fast}; (d) Results from CPD(non-rigid)~\cite{myronenko2010point}; (e) Results from PointPWC-Net(\textit{w/o ft+Full}) that is trained with supervision on FlyingThings3D, and directly evaluate on KITTI without any fine-tuning; (f) Results from PointPWC-Net(\textit{w/ ft + Self + Self}) which is trained on FlyingThings3D and fine-tuned on KITTI using the proposed self-supervised loss. Red ellipses indicate locations with significant non-rigid motion. Enlarge images for better view. (Best viewed in color)}
    \label{fig:res_kitti}
\end{figure}


\noindent \textbf{Train and Evaluate on FlyingThings3D.}
We can see that our PointPWC-Net outperforms traditional methods on all the metrics with a large margin. See Fig.\ref{fig:res_flyingthings3d}(f) for example results. 

\noindent \textbf{Evaluate on KITTI w/o Fine-tuning.}
Even only trained on FlyingThings3D without ground truth labels, our method can obtain  $\mathit{0.2549m}$ on \textit{EPE3D} on KITTI, which improves over CPD(non-rigid) by $\mathit{38.5\%}$, FGR(rigid) by $\mathit{47.3\%}$, and ICP(rigid) by $\mathit{50.8\%}$. %One interesting result is that our PointPWC-Net trained without ground truth is able to outperform SPLATFlowNet trained with ground truth flow on \textit{Acc3DS}. 

\noindent \textbf{Fine-tune on KITTI.} 
With proposed self-supervised loss, we are able to fine-tune the FlyingThings3D trained models on KITTI without using any ground truth. In Table~\ref{tab:results}, the row \textit{PointPWC-Net(w/ ft) Full+Self} and \textit{PointPWC-Net(w/ ft) Self+Self} show the results. \textit{Full+Self} means the model is trained with supervision on FlyingThings3D, then fine-tuned on KITTI without supervision. \textit{Self+Self} means the model is firstly trained on FlyingThings3D, then fine-tuned on KITTI both using self-supervised loss. With KITTI fine-tuning, our PointPWC-Net can achieve \textit{EPE3D} $< 5cm$. Especially, our \textit{PointPWC-Net(w/ ft) Self+Self}, which is fully trained without any ground truth information, achieves similar performance on KITTI as the one that utilized FlyingThings3D ground truth. See Fig.\ref{fig:res_kitti}(f) for example results. 

\subsection{Ablation Study}\label{sec:ablation}
We further conduct ablation studies on model design choices and the self-supervised loss function. On model design, we evaluate the different choices of cost volume layer and removing the warping layer.
%, and removing the concatenation of the global feature and the feature from scene flow predictor. 
On the loss function, we investigate removing the smoothness constraint and Laplacian regularization in the self-supervised learning loss. All models in the ablation studies are trained using FlyingThings3D, and tested on the FlyingThings3D evaluation dataset.


\begin{table}[t]
\centering
%\raggedleft
%\footnotesize
\begin{minipage}[t]{0.48\linewidth}
    \centering
    \caption{\textbf{Loss functions.} The Chamfer loss is not enough to estimate a good scene flow. With the smoothness constraint, the scene flow result improves by $38.2\%$. Laplacian regularization also improves slightly}\label{tab:lossfunction}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{c|c|c|c}
        \hline
        Chamfer & Smoothness & Laplacian & EPE3D(m)$\downarrow$ \\
        \noalign{\smallskip}\hline\noalign{\smallskip}
        \checkmark&  -    &   -   & 0.2112 \\
        \checkmark&\checkmark&  -   &  0.1304 \\
        \checkmark&\checkmark&\checkmark&  \textbf{0.1213} \\
        \noalign{\smallskip}\hline
        \end{tabular}
    }
\end{minipage}
%\hspace{0.2cm}
\begin{minipage}[t]{0.48\linewidth}
    %\begin{table}[t]
    %\raggedleft
    %\footnotesize
    \centering
    \caption{\textbf{Runtime.} Average runtime(ms) on Flyingthings3D. The runtime for FlowNet3D and HPLFlowNet is reported from \cite{gu2019hplflownet} on a single Titan V. The runtime for our PointPWC-Net is reported on a single 1080Ti}\label{tab:runtime}
    \resizebox{0.7\columnwidth}{!}{
        \begin{tabular}{l|c}
        \hline\noalign{\smallskip}
        Method      & Runtime(ms)$\downarrow$ \\
        \noalign{\smallskip}\hline\noalign{\smallskip}
        FlowNet3D~\cite{liu2019flownet3d} & 130.8 \\
        HPLFlowNet~\cite{gu2019hplflownet} & 98.4\\
        PointPWC-Net & 117.4 \\
        \noalign{\smallskip}\hline
        \end{tabular}
    }
\end{minipage}%
\end{table}

Tables~\ref{tab:modeldesign}%,~\ref{tab:features}
,~\ref{tab:lossfunction} show the results of the ablation studies. In Table~\ref{tab:modeldesign} we can see that our design of the cost volume obtains significantly better results than the inner product-based cost volume in PWC-Net~\cite{sun2018pwc} and FlowNet3D~\cite{liu2019flownet3d}, and the warping layer is crucial for performance.
%Table.~\ref{tab:features} shows the upsampled and concatenated global and predictor features from one level coarser both significantly improve the performance over not having the concatenation links.
In Table~\ref{tab:lossfunction}, we see that both the smoothness constraint and Laplacian regularization improve the performance in self-supervised learning. In Table~\ref{tab:runtime}, we report the runtime of our PointPWC-Net, which is comparable with other deep learning based methods and much faster than traditional ones. %Table~\ref{tab:runtime_breakdown} includes the runtime of each critical component in PointPWC-Net.

\begin{comment}
\begin{table}
\centering
\begin{tabular}{c|c|c}
\hline\noalign{\smallskip}
Sup. & Finetune with self-supervision & EPE3D$\downarrow$   \\ 
\noalign{\smallskip}\hline\noalign{\smallskip}
\multirow{2}{*}{$\mathit{Full}$} &    -    & 0.0694  \\
           &        \checkmark             & \textbf{0.0415}  \\ 
\noalign{\smallskip}\hline\noalign{\smallskip}
\multirow{2}{*}{$\mathit{Self}$} &   -      & 0.2549  \\ 
             &        \checkmark            & \textbf{0.0457} \\ 
\noalign{\smallskip}\hline
\end{tabular}
\caption{\textbf{Fine-tuning with self-supervised loss on KITTI.} With proposed self-supervised loss, we are able to finetune the FlyingThings3D trained models on KITTI without using the knowledge of ground truth label. $\mathit{Full}$ means the model is pretrained using fully-supervised loss on FlyingThings3D. $\mathit{Self}$ means the model is pretrained using self-supervised loss on FlyingThings3D. Both models give significantly better results with fine-tuning on KITTI using self-supervised loss}
\label{tab:finetune}
\end{table}
\end{comment}


==> Segment any RGBD/tex/0_abstract.tex <==
\begin{abstract}

The Segment Anything Model (SAM) has demonstrated its effectiveness in segmenting any part of 2D RGB images. However, SAM exhibits a stronger emphasis on texture information while paying less attention to geometry information when segmenting RGB images. To address this limitation, we propose the Segment Any RGBD (SAD) model, which is specifically designed to extract geometry information directly from images. Inspired by the natural ability of humans to identify objects through the visualization of depth maps, SAD utilizes SAM to segment the rendered depth map, thus providing cues with enhanced geometry information and mitigating the issue of over-segmentation. We further include the open-vocabulary semantic segmentation in our framework, so that the 3D panoptic segmentation is fulfilled.
The project is available on \href{https://github.com/Jun-CEN/SegmentAnyRGBD}{https://github.com/Jun-CEN/SegmentAnyRGBD}.

\end{abstract}

==> Segment any RGBD/tex/1_introduction.tex <==
\section{Introduction}
Recently, a prominent model for image segmentation called the Segment Anything model (SAM) has been introduced~\cite{kirillov2023segment}. SAM serves as a robust foundation model for effectively segmenting 2D images in various scenarios.
However, during the segmentation of 2D RGB images, it has been observed that SAM primarily relies on texture information, such as color, leading to over-segmentation results. Consequently, the challenge lies in finding a way to obtain segmentation results that incorporate more geometric information through the utilization of SAM.

To address this issue, we draw inspiration from the remarkable ability of humans to identify objects by visualizing depth maps.
We first map a depth map ($\mathbb{R}^{H\times W}$) to the RGB space ($\mathbb{R}^{H\times W\times 3}$) by a colormap function and then feed the rendered depth image into SAM. Compared to RGB images, the rendered depth image ignores the texture information and focuses on the geometry information, as shown in Fig.~\ref{fig:example}. Notably, it is worth mentioning that while previous SAM-based projects~\cite{zhang2023comprehensive} like SSA~\cite{SSA}, Anything-3D~\cite{shen2023anything3d}, and SAM 3D~\cite{pointcept2023} primarily employ RGB images as inputs, we are the first to utilize SAM for directly segmenting rendered depth images.

==> Segment any RGBD/tex/2_method.tex <==
\section{Method}

\begin{figure}[h]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figs/flowchart_2.png}
         \vspace{-10pt}
		\caption{\textbf{The overview of the proposed SAD.} }
        \vspace{-10pt}
		\label{fig:flowchart}
	\end{center}
\end{figure}

\subsection{Preliminaries}
\textbf{Segment Anything Model (SAM).} The Segment Anything model (SAM)~\cite{kirillov2023segment} is a recently developed large Vision Transformer (ViT)-based model. SAM has been trained on an extensive visual corpus known as SA-1B. The training process on this large-scale dataset has endowed SAM with the remarkable ability to perform zero-shot segmentation on diverse styles of 2D images.

\textbf{Open-Vocabulary Semantic Segmentation (OVSeg).} Given the class candidates in the text format, Open-Vocabulary Semantic Segmentation (OVSeg)~\cite{liang2022open} can segment an image into semantic regions even if the categories are not seen during training.

\subsection{Segment Any RGBD}
% In our project, we provide two alternatives for the users, including feeding the RGB images or rendered depth images to the SAM. In each mode, the user could obtain the semantic masks (one color refers to one class) and the SAM masks with the class. The overall structure is shown in Fig.~\ref{fig:flowchart}. We use OVSeg for zero-shot semantic segmentation.
In this paper, we propose Segment Any RGBD (SAD) that leverages both SAM and OVSeg to achieve semantic segmentation results utilizing the geometry information derived from depth maps.
The overview of SAD is shown in Fig.~\ref{fig:flowchart}. The process can be divided into the following parts:

\textbf{Rendering depth maps.} We notice that depth maps tend to emphasize geometry information over texture information when compared to RGB images, as visually depicted in Fig.~\ref{fig:example}. Capitalizing on this characteristic, our approach involves initially utilizing a colormap function~\cite{Hunter:2007} to render the depth maps to the RGB space. We try different colormaps such as Viridis, Gray, Plasma, Cividis, and Purples, as shown in Fig.~\ref{fig:example}. Consequently, the rendered depth maps are employed as inputs for SAM.

\textbf{Segmentation with SAM.} Following the rendering process, we apply SAM to the rendered depth images to generate initial SAM masks. It is worth noting that these initial SAM masks are class-agnostic and still over-segmented, as illustrated in the Fig.~\ref{fig:example}.

\textbf{Semantic segmentation with OVSeg.} By employing RGB images as input and leveraging text prompts, OVSeg exhibits the ability to generate coarse masks that encompass significant semantic information. These coarse semantic segmentation masks serve a dual role: firstly, they assist in guiding the clustering process of the over-segmented parts within the SAM masks, and secondly, they provide crucial category insights that contribute to refining the fine-grained SAM results.

\textbf{Semantic voting.} For each pixel in the SAM mask, we first find its corresponding predicted class from the OVSeg mask. Subsequently, we assign the class of each segment based on the majority class of pixels contained within it.
Following this, we can proceed to cluster adjacent segments that belong to the same class.

Finally, the semantic segmentation results can be projected to 3D-world based on the depth map for stereoscopic visualizations. This projection enables a comprehensive understanding and visual representation of the segmented results in their spatial context.


==> Segment any RGBD/tex/3_comparision.tex <==
\section{Comparison with RGB Image Input}
We compare the proposed rendered depth image input with the RGB image input.
RGB images predominantly capture texture information, while depth images primarily contain geometry information. As a result, RGB images tend to be more vibrant and colorful compared to the rendered depth images. Consequently, SAM produces a larger number of masks for RGB inputs compared to depth inputs, as illustrated in Fig.~\ref{fig:comparison}.
The utilization of rendered depth images mitigates the issue of over-segmentation in SAM. For instance, when examining the table, the RGB images segment it into four distinct parts, with one part being misclassified as a chair in the semantic results (indicated by yellow circles in Fig.\ref{fig:comparison}), while it is accurately classified in the depth image.
It is also important to note that when two objects are in close proximity, they may be segmented as a single object in the depth image, as depicted by the chair in the red circle of Fig.~\ref{fig:comparison}. In such cases, the texture information present in RGB images becomes crucial for accurately identifying and distinguishing the objects.

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figs/comparison.png}
         \vspace{-10pt}
		\caption{\textbf{Segmentation results with the RGB image input and the rendered depth image inputs.} }
        \vspace{-10pt}
		\label{fig:comparison}
	\end{center}
\end{figure}

==> Segment any RGBD/tex/4_experiments.tex <==
\section{Qualitative Results}
We present qualitative results on Sailvos3D~\cite{HuCVPR2021} and ScanNet~\cite{dai2017scannet}, which are depicted in Fig.~\ref{fig:sailvos3D} and Fig.~\ref{fig:scannet}. The figures clearly demonstrate the enhanced performance of our method in generating geometric semantic segmentation results when utilizing depth map inputs.

\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figs/qualitative_results_sailvos3D.pdf}
         \vspace{-10pt}
		\caption{\textbf{Qualitative results on the Sailvos3D dataset.}}
        \vspace{-10pt}
		\label{fig:sailvos3D}
	\end{center}
\end{figure}

\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{Figs/qualitative_results_scannet.pdf}
         \vspace{-10pt}
		\caption{\textbf{Qualitative results on the ScannetV2 dataset.}}
        \vspace{-10pt}
		\label{fig:scannet}
	\end{center}
\end{figure}

==> Segment any RGBD/tex/conclusions.tex <==
\section{Conclusion}
In summary, we introduce the Segment Any RGBD (SAD) model, which combines SAM and OVSeg for semantic segmentation using depth maps. SAD leverages the geometry information of depth maps by rendering them with RGB information and feeding them into SAM. Initial SAM masks are generated, which are refined using OVSeg's coarse semantic segmentation masks.
The clustering process is then applied to group adjacent segments of the same class, improving the segmentation results' coherence. Finally, the semantic segmentation results are projected onto the 3D world based on the depth map, enabling comprehensive stereoscopic visualization.
Overall, SAD enhances semantic segmentation by incorporating depth maps and leveraging both SAM and OVSeg, resulting in more accurate and context-aware segmentation results. This work opens up new possibilities for advancing semantic segmentation tasks and provides valuable insights into real-world applications.


==> exp.tex <==
\begin{table}[t]
    \centering
    \caption{\textbf{Evaluation results on the FlyingThings3D and KITTI datasets.} $\mathit{Self}$ means self-supervised, $\mathit{Full}$ means fully-supervised. All approaches are (at least) trained on FlyingThings3D. On KITTI, $\mathit{Self}$ and $\mathit{Full}$ refer to the respective models trained on FlyingThings3D that is directly evaluated on KITTI, while \textit{Self+Self} means the model is firstly trained on FlyingThings3D with self-supervision, then fine-tuned on KITTI  with self-supervision as well. \textit{Full+Self} means the model is trained with full supervision on FlyingThings3D, then fine-tuned on KITTI with self-supervision. ICP~\cite{besl1992method}, FGR~\cite{zhou2016fast}, and CPD~\cite{myronenko2010point} are traditional method that does not require training. Our model outperforms all baselines by a large margin on all metrics}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|l|c|cccc|cc}
        %\cline{2-9}
        \hline\noalign{\smallskip}
        Dataset &Method         & Sup.  & EPE3D(m)$\downarrow$           & Acc3DS$\uparrow$          & Acc3DR$\uparrow$          & Outliers3D$\downarrow$      & EPE2D(\textit{px})$\downarrow$           & Acc2D$\uparrow$           \\
        \noalign{\smallskip}\hline\noalign{\smallskip}
    \multirow{9}{*}{Flyingthings3D}&ICP(rigid)~\cite{besl1992method} & $\mathit{Self}$& 0.4062          & 0.1614          & 0.3038          & 0.8796          & 23.2280         & 0.2913          \\
        &FGR(rigid)~\cite{zhou2016fast}        &$\mathit{Self}$& 0.4016  & 0.1291   & 0.3461  & 0.8755  & 28.5165  & 0.3037    \\
        &CPD(non-rigid)~\cite{myronenko2010point} &$\mathit{Self}$& 0.4887  & 0.0538   & 0.1694  & 0.9063  & 26.2015  & 0.0966    \\
        &PointPWC-Net   & $\mathit{Self}$& \textbf{0.1213} & \textbf{0.3239} & \textbf{0.6742} & \textbf{0.6878} & \textbf{6.5493} & \textbf{0.4756} \\
        \noalign{\smallskip}\cline{2-9}\noalign{\smallskip}
        &FlowNet3D~\cite{liu2019flownet3d}     &$\mathit{Full}$& 0.1136          & 0.4125          & 0.7706          & 0.6016          & 5.9740          & 0.5692          \\
        &SPLATFlowNet~\cite{su2018splatnet}   &$\mathit{Full}$& 0.1205          & 0.4197          & 0.7180          & 0.6187          & 6.9759          & 0.5512          \\
        &original BCL~\cite{gu2019hplflownet}   &$\mathit{Full}$& 0.1111          & 0.4279          & 0.7551          & 0.6054          & 6.3027          & 0.5669          \\
        &HPLFlowNet~\cite{gu2019hplflownet}     &$\mathit{Full}$& 0.0804          & 0.6144          & 0.8555          & 0.4287 & 4.6723          & 0.6764          \\
        &PointPWC-Net   &$\mathit{Full}$& \textbf{0.0588} & \textbf{0.7379} & \textbf{0.9276} & \textbf{0.3424}  & \textbf{3.2390} & \textbf{0.7994} \\
        \noalign{\smallskip}\hline\noalign{\smallskip}
    \multirow{11}{*}{KITTI}&ICP(rigid)~\cite{besl1992method}        &$\mathit{Self}$& 0.5181          & 0.0669          & 0.1667          & 0.8712          & 27.6752         & 0.1056          \\
        &FGR(rigid)~\cite{zhou2016fast}        &$\mathit{Self}$& 0.4835  & 0.1331   & 0.2851  & 0.7761  & 18.7464  & 0.2876    \\
        &CPD(non-rigid)~\cite{myronenko2010point}        &$\mathit{Self}$& 0.4144  & 0.2058      & 0.4001 & 0.7146 & 27.0583 & 0.1980 \\
        &PointPWC-Net(w/o ft) &$\mathit{Self}$& \textit{0.2549} & \textit{0.2379} & \textit{0.4957} & \textit{0.6863} & \textit{8.9439} & \textit{0.3299} \\
        &PointPWC-Net(w/ ft) &$\mathit{Self + Self}$& \textbf{0.0461} & \textbf{0.7951} & \textbf{0.9538} & \textbf{0.2275} & \textbf{2.0417} & \textbf{0.8645} \\
        \noalign{\smallskip}\cline{2-9}\noalign{\smallskip}
        &FlowNet3D~\cite{liu2019flownet3d}   &$\mathit{Full}$& 0.1767          & 0.3738          & 0.6677          & 0.5271          & 7.2141          & 0.5093          \\
        &SPLATFlowNet~\cite{su2018splatnet} &$\mathit{Full}$& 0.1988          & 0.2174          & 0.5391          & 0.6575          & 8.2306          & 0.4189          \\
        &original BCL~\cite{gu2019hplflownet} &$\mathit{Full}$& 0.1729          & 0.2516          & 0.6011          & 0.6215          & 7.3476          & 0.4411          \\
        &HPLFlowNet~\cite{gu2019hplflownet}   &$\mathit{Full}$& 0.1169 & 0.4783          & 0.7776 & 0.4103          & 4.8055          & 0.5938          \\
        &PointPWC-Net(w/o ft) &$\mathit{Full}$& \textit{0.0694}  & \textit{0.7281} & \textit{0.8884} & \textit{0.2648} & \textit{3.0062} & \textit{0.7673} \\
        &PointPWC-Net(w/ ft) &$\mathit{Full+Self}$& \textbf{0.0430} & \textbf{0.8175} & \textbf{0.9680} & \textbf{0.2072} & \textbf{1.9022} & \textbf{0.8669} \\
        \noalign{\smallskip}\hline
    \end{tabular}
    \label{tab:results}
    }
\end{table}


In this section, we train and evaluate our PointPWC-Net on the FlyingThings3D dataset~\cite{mayer2016large} with the supervised loss and the self-supervised loss, respectively. Then, we evaluate the generalization ability of our model by first applying the model on the real-world KITTI Scene Flow dataset~\cite{Menze2018JPRS,Menze2015ISA} \textit{without any fine-tuning}. Then, with the proposed self-supervised losses, we further fine-tune our pre-trained model on the KITTI dataset to study the best performance we could obtain without supervision. Besides, we also compare the runtime of our model with previous work. Finally, we conduct ablation studies to analyze the contribution of each part of the model and the loss function.

\noindent \textbf{Implementation Details.} We build a 4-level feature pyramid from the input point cloud. The weights $\alpha$ are set to be $\alpha_0=0.02$, $\alpha_1=0.04$, $\alpha_2=0.08$, and $\alpha_3=0.16$, with weight decay $0.0001$.% for both supervised learning and self-supervised learning. 
The scale factor $\beta$ in self-supervised learning are set to be $\beta_1=1.0$, $\beta_2=1.0$, and $\beta_3=0.3$. We train our model starting from a learning rate of $0.001$ and reducing by half every 80 epochs. All the hyperparameters are set using the validation set of FlyingThings3D with 8,192 points in each input point cloud.

\noindent \textbf{Evaluation Metrics.} For fair comparison, we adopt the evaluation metrics that are used in \cite{gu2019hplflownet}. Let $SF_{\Theta}$ denote the predicted scene flow, and $SF_{GT}$ be the ground truth scene flow. The evaluate metrics are computed as follows:

\noindent $\bullet$ \textit{EPE3D(m)}: $\norm{SF_{\Theta}-SF_{GT}}_2$ averaged over each point in meters.

\noindent $\bullet$ \textit{Acc3DS}: the percentage of points with \textit{EPE3D} $< 0.05m$ or relative error $<5\%$.

\noindent $\bullet$ \textit{Acc3DR}: the percentage of points with \textit{EPE3D} $< 0.1m$ or relative error $<10\%$.

\noindent $\bullet$ \textit{Outliers3D}: the percentage of points with \textit{EPE3D}$>0.3m$ or relative error $>10\%$.

\noindent $\bullet$ \textit{EPE2D(px)}: 2D end point error obtained by projecting point clouds back to the image plane.

\noindent $\bullet$ \textit{Acc2D}: the percentage of points whose \textit{EPE2D} $< 3px$ or relative error $<5\%$.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{images/fly_compare.pdf}
    \caption{\textbf{Results on the FlyingThings3D dataset.} In (a), 2 point clouds PC1 and PC2 are presented in Magenta and Green, respectively. In (b-f), PC1 is warped to PC2 based on the (computed) scene flow. (b) shows the ground truth; (c) Results from FGR(rigid)~\cite{zhou2016fast}; (d) Results from CPD(non-rigid)~\cite{myronenko2010point}; (e) Results from PointPWC-Net(\textit{Full}); (f) Results from PointPWC-Net(\textit{Self}). Red ellipses indicate locations with significant non-rigid motion. Enlarge images for better view. (Best viewed in color)}
    \label{fig:res_flyingthings3d}
\end{figure}

\subsection{Supervised Learning}
First we conduct experiments with supervised loss. To our knowledge, there is no publicly available large-scale real-world dataset that has scene flow ground truth from point clouds (The input to the KITTI scene flow benchmark is 2D), thus we train our PointPWC-Net on the synthetic Flyingthings3D dataset, following~\cite{gu2019hplflownet}. Then, the pre-trained model is directly evaluated on KITTI Scene Flow 2015 dataset without any fine-tuning. % to demonstrate the generalization ability of our model.


\noindent \textbf{Train and Evaluate on FlyingThings3D.}
The FlyingThings3D training dataset includes 19,640 pairs of point clouds, and the evaluation dataset includes 3,824 pairs of point clouds. Our model takes $n=8,192$ points in each point cloud. We first train the model with $\frac{1}{4}$ of the training set(4,910 pairs), and then fine-tune it on the whole training set, to speed up training.

Table~\ref{tab:results} shows the quantitative evaluation results on the Flyingthings3D dataset. 
%We compare our method with FlowNet3D~\cite{liu2019flownet3d}, SPLATFlowNet~\cite{su2018splatnet}, original BCL~\cite{gu2019hplflownet}, and HPLFlowNet~\cite{gu2019hplflownet}. 
Our method outperforms all the methods on all metrics by a large margin. %Compared to FlowNet3D, our cost volume layer is able to capture the motion information better. 
Comparing to SPLATFlowNet, original BCL, and HPLFlowNet, our method avoids the preprocessing step of building a permutohedral lattice from the input. Besides, our method outperforms HPLFlowNet on \textit{EPE3D} by $\mathit{26.9\%}$. And, we are the only method with \textit{EPE2D} under 4px, which improves over HPLFlowNet by $\mathit{30.7\%}$. See Fig.\ref{fig:res_flyingthings3d}(e) for example results.

\noindent \textbf{Evaluate on KITTI w/o Fine-tune.} To study the generalization ability of our PointPWC-Net, we directly take the model trained using FlyingThings3D and evaluate it on KITTI Scene Flow 2015~\cite{Menze2015ISA,Menze2018JPRS} \textit{without any fine-tuning}. KITTI Scene Flow 2015 consists of 200 training scenes and 200 test scenes. To evaluate our PointPWC-Net, we use  ground truth labels and trace raw point clouds associated with the frames, following \cite{liu2019flownet3d,gu2019hplflownet}. Since no point clouds and ground truth are provided on test set, we evaluate on all 142 scenes in the training set with available point clouds. We remove ground points with height $<0.3m$ following \cite{gu2019hplflownet} for fair comparison with previous methods. 

From Table~\ref{tab:results}, our PointPWC-Net outperforms all the state-of-the-art methods, which demonstrates the generalization ability of our model. For \textit{EPE3D}, our model is the only one below $10cm$, which improves over HPLFlowNet by $\mathit{40.6\%}$. For \textit{Acc3DS}, our method outperforms both FlowNet3D and HPLFlowNet by $\mathit{35.4\%}$ and $\mathit{25.0\%}$ respectively. See Fig.\ref{fig:res_kitti}(e) for example results. 

\begin{table}[t]
    \centering
    \caption{\textbf{Model design.} A learnable cost volume preforms much better than inner product cost volume used in PWC-Net~\cite{sun2018pwc}. Using our cost volume instead of the MLP+Maxpool used in FlowNet3D's flow embedding layer improves performance by $20.6\%$. Compared to no warping, the warping layer improves the performance by $40.2\%$}
    \begin{tabular}{l|c|c}
    \hline\noalign{\smallskip}
    Component                      & Status & EPE3D(m)$\downarrow$ \\
    \noalign{\smallskip}\hline\noalign{\smallskip}
    \multirow{3}{*}{Cost Volume}   & PWC-Net~\cite{sun2018pwc}& 0.0821 \\
                                   & MLP+Maxpool(learnable)~\cite{liu2019flownet3d}& 0.0741 \\
                                   & Ours(learnable) &  \textbf{0.0588} \\
    \noalign{\smallskip}\hline\noalign{\smallskip}
    \multirow{2}{*}{Warping Layer} & w/o      & 0.0984 \\
                                   & w    & \textbf{0.0588} \\
    \noalign{\smallskip}\hline
    \end{tabular}
    \label{tab:modeldesign}
\end{table}

\subsection{Self-supervised Learning}
Acquiring or annotating dense scene flow from real-world 3D point clouds is very expensive, so it would be interesting to evaluate the performance of our self-supervised approach. %study how to estimate scene flow given two input point clouds without ground truth. Based on the observation that the input point clouds should have structure or shape correspondences, %we propose to use Chamfer distance along with smoothness constraint and Laplac
%ian regularization as loss function to estimate scene flow. 
We train our model using the same procedure as in supervised learning, i.e. first train the model with one quarter of the training dataset, then fine-tune with the whole training set. Table~\ref{tab:results} gives the quantitative results on PointPWC-Net with self-supervised learning. We compare our method with ICP(rigid)~\cite{besl1992method}, FGR(rigid)~\cite{zhou2016fast} and CPD(non-rigid)~\cite{myronenko2010point}. Because traditional point registration methods are not trained with ground truth, we can view them as self/un-supervised methods. 



\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{images/kitti_compare.pdf}
    \caption{\textbf{Results on the KITTI Scene Flow 2015 dataset.} In (a), 2 point clouds PC1 and PC2 are presented in Magenta and Green, respectively. In (b-f), PC1 is warped to PC2 based on the (computed) scene flow. (b) shows the ground truth; (c) Results from FGR(rigid)~\cite{zhou2016fast}; (d) Results from CPD(non-rigid)~\cite{myronenko2010point}; (e) Results from PointPWC-Net(\textit{w/o ft+Full}) that is trained with supervision on FlyingThings3D, and directly evaluate on KITTI without any fine-tuning; (f) Results from PointPWC-Net(\textit{w/ ft + Self + Self}) which is trained on FlyingThings3D and fine-tuned on KITTI using the proposed self-supervised loss. Red ellipses indicate locations with significant non-rigid motion. Enlarge images for better view. (Best viewed in color)}
    \label{fig:res_kitti}
\end{figure}


\noindent \textbf{Train and Evaluate on FlyingThings3D.}
We can see that our PointPWC-Net outperforms traditional methods on all the metrics with a large margin. See Fig.\ref{fig:res_flyingthings3d}(f) for example results. 

\noindent \textbf{Evaluate on KITTI w/o Fine-tuning.}
Even only trained on FlyingThings3D without ground truth labels, our method can obtain  $\mathit{0.2549m}$ on \textit{EPE3D} on KITTI, which improves over CPD(non-rigid) by $\mathit{38.5\%}$, FGR(rigid) by $\mathit{47.3\%}$, and ICP(rigid) by $\mathit{50.8\%}$. %One interesting result is that our PointPWC-Net trained without ground truth is able to outperform SPLATFlowNet trained with ground truth flow on \textit{Acc3DS}. 

\noindent \textbf{Fine-tune on KITTI.} 
With proposed self-supervised loss, we are able to fine-tune the FlyingThings3D trained models on KITTI without using any ground truth. In Table~\ref{tab:results}, the row \textit{PointPWC-Net(w/ ft) Full+Self} and \textit{PointPWC-Net(w/ ft) Self+Self} show the results. \textit{Full+Self} means the model is trained with supervision on FlyingThings3D, then fine-tuned on KITTI without supervision. \textit{Self+Self} means the model is firstly trained on FlyingThings3D, then fine-tuned on KITTI both using self-supervised loss. With KITTI fine-tuning, our PointPWC-Net can achieve \textit{EPE3D} $< 5cm$. Especially, our \textit{PointPWC-Net(w/ ft) Self+Self}, which is fully trained without any ground truth information, achieves similar performance on KITTI as the one that utilized FlyingThings3D ground truth. See Fig.\ref{fig:res_kitti}(f) for example results. 

\subsection{Ablation Study}\label{sec:ablation}
We further conduct ablation studies on model design choices and the self-supervised loss function. On model design, we evaluate the different choices of cost volume layer and removing the warping layer.
%, and removing the concatenation of the global feature and the feature from scene flow predictor. 
On the loss function, we investigate removing the smoothness constraint and Laplacian regularization in the self-supervised learning loss. All models in the ablation studies are trained using FlyingThings3D, and tested on the FlyingThings3D evaluation dataset.


\begin{table}[t]
\centering
%\raggedleft
%\footnotesize
\begin{minipage}[t]{0.48\linewidth}
    \centering
    \caption{\textbf{Loss functions.} The Chamfer loss is not enough to estimate a good scene flow. With the smoothness constraint, the scene flow result improves by $38.2\%$. Laplacian regularization also improves slightly}\label{tab:lossfunction}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{c|c|c|c}
        \hline
        Chamfer & Smoothness & Laplacian & EPE3D(m)$\downarrow$ \\
        \noalign{\smallskip}\hline\noalign{\smallskip}
        \checkmark&  -    &   -   & 0.2112 \\
        \checkmark&\checkmark&  -   &  0.1304 \\
        \checkmark&\checkmark&\checkmark&  \textbf{0.1213} \\
        \noalign{\smallskip}\hline
        \end{tabular}
    }
\end{minipage}
%\hspace{0.2cm}
\begin{minipage}[t]{0.48\linewidth}
    %\begin{table}[t]
    %\raggedleft
    %\footnotesize
    \centering
    \caption{\textbf{Runtime.} Average runtime(ms) on Flyingthings3D. The runtime for FlowNet3D and HPLFlowNet is reported from \cite{gu2019hplflownet} on a single Titan V. The runtime for our PointPWC-Net is reported on a single 1080Ti}\label{tab:runtime}
    \resizebox{0.7\columnwidth}{!}{
        \begin{tabular}{l|c}
        \hline\noalign{\smallskip}
        Method      & Runtime(ms)$\downarrow$ \\
        \noalign{\smallskip}\hline\noalign{\smallskip}
        FlowNet3D~\cite{liu2019flownet3d} & 130.8 \\
        HPLFlowNet~\cite{gu2019hplflownet} & 98.4\\
        PointPWC-Net & 117.4 \\
        \noalign{\smallskip}\hline
        \end{tabular}
    }
\end{minipage}%
\end{table}

Tables~\ref{tab:modeldesign}%,~\ref{tab:features}
,~\ref{tab:lossfunction} show the results of the ablation studies. In Table~\ref{tab:modeldesign} we can see that our design of the cost volume obtains significantly better results than the inner product-based cost volume in PWC-Net~\cite{sun2018pwc} and FlowNet3D~\cite{liu2019flownet3d}, and the warping layer is crucial for performance.
%Table.~\ref{tab:features} shows the upsampled and concatenated global and predictor features from one level coarser both significantly improve the performance over not having the concatenation links.
In Table~\ref{tab:lossfunction}, we see that both the smoothness constraint and Laplacian regularization improve the performance in self-supervised learning. In Table~\ref{tab:runtime}, we report the runtime of our PointPWC-Net, which is comparable with other deep learning based methods and much faster than traditional ones. %Table~\ref{tab:runtime_breakdown} includes the runtime of each critical component in PointPWC-Net.

\begin{comment}
\begin{table}
\centering
\begin{tabular}{c|c|c}
\hline\noalign{\smallskip}
Sup. & Finetune with self-supervision & EPE3D$\downarrow$   \\ 
\noalign{\smallskip}\hline\noalign{\smallskip}
\multirow{2}{*}{$\mathit{Full}$} &    -    & 0.0694  \\
           &        \checkmark             & \textbf{0.0415}  \\ 
\noalign{\smallskip}\hline\noalign{\smallskip}
\multirow{2}{*}{$\mathit{Self}$} &   -      & 0.2549  \\ 
             &        \checkmark            & \textbf{0.0457} \\ 
\noalign{\smallskip}\hline
\end{tabular}
\caption{\textbf{Fine-tuning with self-supervised loss on KITTI.} With proposed self-supervised loss, we are able to finetune the FlyingThings3D trained models on KITTI without using the knowledge of ground truth label. $\mathit{Full}$ means the model is pretrained using fully-supervised loss on FlyingThings3D. $\mathit{Self}$ means the model is pretrained using self-supervised loss on FlyingThings3D. Both models give significantly better results with fine-tuning on KITTI using self-supervised loss}
\label{tab:finetune}
\end{table}
\end{comment}

